First data from the CUPID-Mo neutrinoless double beta decay experiment

The CUPID-Mo experiment is searching for neutrinoless double beta decay in $^{100}$Mo, evaluating the technology of cryogenic scintillating Li$_{2}^{100}$MoO$_4$ detectors for CUPID (CUORE Upgrade with Particle ID). CUPID-Mo detectors feature background suppression using a dual-readout scheme with Li$_{2}$MoO$_4$ crystals complemented by Ge bolometers for light detection. The detection of both heat and scintillation light signals allows the efficient discrimination of $\alpha$ from $\gamma$&$\beta$ events. In this proceedings, we discuss results from the first 2 months of data taking in spring 2019. In addition to an excellent bolometric performance of 6.7$\,$keV (FWHM) at 2615$\,$keV and an $\alpha$ separation of better than 99.9\% for all detectors, we report on bulk radiopurity for Th and U. Finally, we interpret the accumulated physics data in terms of a limit of $T_{1/2}^{0\nu}\,> 3\times10^{23}\,$yr for $^{100}$Mo and discuss the sensitivity of CUPID-Mo until the expected end of physics data taking in early 2020.

==> authorlist.tex <==
\author{
E.~Armengaud$^1$,
C.~Augier$^2$,
A.~S.~Barabash$^3$,
F.~Bellini$^4, ^5$,
G.~Benato$^6$,
A.~Beno\^{\i}t$^7$,
M.~Beretta$^8, ^9$,
L.~Berg\'e$^{10}$,
J.~Billard$^2$,
Yu.~A.~Borovlev$^{11}$,
Ch.~Bourgeois$^{12}$,
M.~Briere$^{12}$,
V.~B.~Brudanin$^{13}$,
P.~Camus$^7$,
L.~Cardani$^5$,
N.~Casali$^5$,
A.~Cazes$^2$,
M.~Chapellier$^{10}$,
F.~Charlieux$^2$,
M.~de~Combarieu$^{14}$,
I.~Dafinei$^5$,
F.~A.~Danevich$^{15}$,
M.~De~Jesus$^2$,
L.~Dumoulin$^{10}$,
K.~Eitel$^{16}$,
E.~Elkhoury$^2$,
F.~Ferri$^1$,
B.~K.~Fujikawa$^{17}$,
J.~Gascon$^2$,
L.~Gironi$^8, ^9$,
A.~Giuliani$^{10},^{18}$,
V.~D.~Grigorieva$^{11}$,
M.~Gros$^1$,
E.~Guerard$^{12}$,
D.~L.~Helis$^1$,
H.~Z.~Huang$^{19}$,
R.~Huang$^6$,
J.~Johnston$^{20}$,
A.~Juillard$^2$,
H.~Khalife$^{10}$, 
M.~Kleifges$^{21}$,
V.~V.~Kobychev$^{15}$,
Yu.~G.~Kolomensky$^6,^{22}$,
S.I.~Konovalov$^3$,
A.~Leder$^{20}$,
P.~Loaiza$^{12}$,
L.~Ma$^{19}$,
E.~P.~Makarov$^{11}$,
P.~de~Marcillac$^{10}$,
L.~Marini$^6,^{17},^{21}$,
S.~Marnieros$^{10}$,
D.~Misiak$^2$,
X.-F.~Navick$^1$,
C.~Nones$^1$,
V.~Novati$^{10}$,
E.~Olivieri$^{10}$,
J.~L.~Ouellet$^{20}$,
L.~Pagnanini$^8, ^9$,
P.~Pari$^{14}$,
L.~Pattavina$^{21},^{24}$,
B.~Paul$^1$,
M.~Pavan$^8, ^9$,
H.~Peng$^{25}$,
G.~Pessina$^9$,
S.~Pirro$^{23}$,
D.~V.~Poda$^{10},^{15}$
O.~G.~Polischuk$^{15}$,
E.~Previtali$^8, ^9$,
Th.~Redon$^{10}$,
S.~Rozov$^{13}$, 
C.~Rusconi$^{26}$,
V.~Sanglard$^2$,
K.~Sch\"affner$^{23}$,
B.~Schmidt$^{17}$,
Y.~Shen$^{19}$,
V.~N.~Shlegel$^{11}$,
B.~Siebenborn$^{16}$,
V.~Singh$^6$,
S.~Sorbino$^4,^5$,
C.~Tomei$^5$,
V.~I.~Tretyak$^{15}$, 
V.~I.~Umatov$^3$,
L.~Vagneron$^2$,
M.~Vel\'azquez$^{27}$,
M.~Weber$^{21}$,
B.~Welliver$^{17}$,
L.~Winslow$^{20}$,
M.~Xue$^{25}$,
E.~Yakushev$^{13}$,
A.~S.~Zolotarova$^{10}$}

\ead{ beschmidt@lbl.gov}

\address{$^1$IRFU, CEA, Universit\'{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\address{$^2$Univ Lyon, Universit\'{e} Lyon 1, CNRS/IN2P3, IP2I-Lyon, F-69622, Villeurbanne, France}  
\address{$^3$National Research Centre Kurchatov Institute, Institute of Theoretical and Experimental Physics, 117218 Moscow, Russia} 
\address{$^4$Dipartimento di Fisica, Sapienza Universit\`a di Roma, P.le Aldo Moro 2, I-00185, Rome, Italy }
\address{$^5$INFN, Sezione di Roma, P.le Aldo Moro 2, I-00185, Rome, Italy}
\address{$^6$Department of Physics, University of California, Berkeley, California 94720, USA }
\address{$^7$CNRS-N\'eel, 38042 Grenoble Cedex 9, France}
\address{$^8$Dipartimento di Fisica, Universit\`{a} di Milano-Bicocca, I-20126 Milano, Italy }
\address{$^9$INFN, Sezione di Milano-Bicocca, I-20126 Milano, Italy }
\address{$^{10}$CSNSM, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, 91405 Orsay, France}
\address{$^{11}$Nikolaev Institute of Inorganic Chemistry, 630090 Novosibirsk, Russia }
\address{$^{12}$LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, 91898 Orsay, France }
\address{$^{13}$Laboratory of Nuclear Problems, JINR, 141980 Dubna, Moscow region, Russia }
\address{$^{14}$IRAMIS, CEA, Universit\'{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France }
\address{$^{15}$Institute for Nuclear Research, 03028 Kyiv, Ukraine }
\address{$^{16}$Karlsruhe Institute of Technology, Institut f\"{u}r Kernphysik, 76021 Karlsruhe, Germany }
\address{$^{17}$Nuclear Science Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA }
\address{$^{18}$DISAT, Universit\`a dell'Insubria, 22100 Como, Italy }
\address{$^{19}$Key Laboratory of Nuclear Physics and Ion-beam Application (MOE), Fudan University, Shanghai 200433, PR China }
\address{$^{20}$Massachusetts Institute of Technology, Cambridge, MA 02139, USA }
\address{$^{21}$Karlsruhe Institute of Technology, Institut f\"{u}r Prozessdatenverarbeitung und Elektronik, 76021 Karlsruhe, Germany}
\address{$^{22}$Physics Division, Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA }
\address{$^{23}$INFN, Laboratori Nazionali del Gran Sasso, I-67100 Assergi (AQ), Italy}
\address{$^{24}$Physik Department, Technische Universit\"at M\"unchen, Garching D-85748, Germany }
\address{$^{25}$Department of Modern Physics, University of Science and Technology of China, Hefei 230027, PR China }
\address{$^{26}$Department of Physics and Astronomy, University of South Carolina, SC 29208, Columbia, USA} 
\address{$^{27}$Universit\'e Grenoble Alpes, CNRS, Grenoble INP, SIMAP, 38402 Saint Martin d'H\'eres, France }
 

